Online Degree-Bounded Steiner Network Design

We initiate the study of degree-bounded network design problems in the online setting. The degree-bounded Steiner tree problem { which asks for a subgraph with minimum degree that connects a given set of vertices { is perhaps one of the most representative problems in this class. This paper deals with its well-studied generalization called the degree-bounded Steiner forest problem where the connectivity demands are represented by vertex pairs that need to be individually connected. In the classical online model, the input graph is given online but the demand pairs arrive sequentially in online steps. The selected subgraph starts off as the empty subgraph, but has to be augmented to satisfy the new connectivity constraint in each online step. The goal is to be competitive against an adversary that knows the input in advance. We design a simple greedy-like algorithm that achieves a competitive ratio of O(log n) where n is the number of vertices. We show that no (randomized) algorithm can achieve a (multiplicative) competitive ratio o(log n); thus our result is asymptotically tight. We further show strong hardness results for the group Steiner tree and the edge-weighted variants of degree-bounded connectivity problems. Fourer and Raghavachari resolved the online variant of degree-bounded Steiner forest in their paper in SODA'92. Since then, the natural family of degree-bounded network design problems has been extensively studied in the literature resulting in the development of many interesting tools and numerous papers on the topic. We hope that our approach in this paper, paves the way for solving the online variants of the classical problems in this family of network design problems.

==> draft (1)/alg.tex <==
\section{Online Degree-Bounded Steiner Forest}\label{sec:sfalg}
Consider an arbitrary online step where a new demand $(s,t)$ arrived. Let
$H$ denote the online output of the previous step.
%and let $CC(H)$ denote the collection of connected components of $H$.
In order to augment $H$ for connecting $s$ and $t$, one can shortcut through
the connected components of $H$. We say an edge $e=(u,v)$ is an
\textit{extension edge} w.r.t. $H$, if $u$ and $v$ are not connected in $H$. Let
$P$ denote an $(s,t)$-path in $G$. The extension part $P^*$ of $P$ is defined
as the set of extension edges of $P$. Observe that augmenting $H$ with $P^*$
satisfies the demand $(s,t)$. For a vertex $v$, we define
$\ell^+_H(v)=\ell_H(v)+{2}/{b_v}$ to be the \textit{uptick load of $v$}. 
We slightly misuse the notation by defining $\ell^+_H(P^*)=\max_{v \in
  V(P^*)} \ell^+_H(v)$ as the uptick load of $P^*$, where $V(P^*)$ is the set of
endpoints of edges in $P^*$.

The \textit{greedy algorithm} (GA) starts with an empty subset $H$. Upon 
arrival of the $i$-{th} demand $(s_i,t_i)$, we find a path $P_i$ with 
smallest uptick load $\ell^+_H(P_i^*)$ where $P_i^*$ is the extension part of
$P_i$. We break ties in favor of the path with a smaller number of edges.
Note that the path $P_i$ can be found efficiently using Dijkstra-like
algorithms. We define $\tau_i=\ell^+_H(P_i^*)$ to be the \textit{arrival threshold}
of the $i$-{th} demand. We satisfy the new demand by adding $P_i^*$ to the edge
set of $H$ (see Algorithm~\ref{alg:dbsf}).

\subsection{Analysis}
%\paragraph{Analysis.} 
We now use a dual-fitting approach to show that GA has an
asymptotically tight competitive ratio of $O(\log(n))$. 
In the following we  use \alg{} to also refer to the \emph{final output}
of our greedy algorithm.
%We also use \alg{} to denote the final output of the greedy algorithm GA.}
%Let \alg{} denote the
%\textit{final output} of GA. 
We first show several structural properties of
\alg{}. We then use these combinatorial properties to construct a family of
feasible dual vectors for \ref{LP:dualsf}. We finally show that there always
exists a member of this family with an objective value of at least a
${1}/{O(\log(n))}$ fraction of the maximum load of a vertex in \alg{}. This
in turn proves the desired competitive ratio by using weak duality.

For a real value $r\geq 0$, let $\Gamma(r)$ denote the set of vertices with
$\ell^+_{\alg}(v)\geq r$. Let $D(r)$ denote the indices of demands $i$ for
which the arrival threshold $\tau_i$ is at least $r$. For a subgraph $X$, let
$\CC(X)$ denote the collection of connected components of $X$. For ease of
notation, we may use the name of a subgraph to denote the set of vertices of
that subgraph as well. Furthermore, for a graph $X$ and a subgraph $Y\subseteq
X$, let $X\setminus Y$ denote the graph obtained from $X$ by removing the
vertices of $Y$.

Recall that $\Mc{S}$ is the collection of subsets that separate the endpoints
of at least one demand. The following lemma, intuitively speaking, implies that
$\Gamma(r)$ well-separates the endpoints of $D(r)$.

\begin{lemma}\label{lem:multiwaycut}
For any threshold $r> 0$, we have
$\left| \CC(G\setminus\Gamma(r)) \cap \Mc{S}  \right| \geq |D(r)|+1 $.
%\hrnote{I don't like this notation but I don't have a better suggestion}
\end{lemma}
\begin{proof}
  For a vertex $v\in G\setminus\Gamma(r)$ we use $\operatorname{CC}(v)$ to
  denote its connected component. Observe that, since the endpoints of demands
  are nodes with infinite degree bound, the endpoints are \emph{not} contained in $\Gamma(r)$, and, hence, are
  in $G\setminus\Gamma(r)$.

  We construct a graph $F$ that has one node for every connected component in
  $G\setminus\Gamma(r)$ that contains an endpoint of a demand in $D(r)$. Edges
  in $F$ are defined as follows. For every demand $i\in D(r)$ between $s_i$ and
  $t_i$, we add an edge that connects the components $\operatorname{CC}(s_i)$
  and $\operatorname{CC}(t_i)$. In the following we argue that $F$ does not
  contain cycles. This gives the lemma since in a forest $|D(r)|+1=|E_F|+1\le|V_F|\le 
  |\CC(G\setminus\Gamma(r)) \cap \Mc{S}|$.

  Assume for contradiction that the sequence $(e_{i_0},\dots,e_{i_{k-1}})$,
  $k\ge 2$ forms a (minimal) cycle in $F$, where $e_{i_j}$ corresponds to the
  demand between vertices $s_{i_j}$ and $t_{i_j}$ (see Figure~\ref{fig:lemsep}
  in the Appendix). Assume wlog.\ that $e_{i_{k-1}}$ is the edge of the cycle for
  which the corresponding demand appears last, i.e., $i_{k-1}\geq i_j$ for
  every $j<k$. Let $H$ denote the online solution at the time of arrival of the
  demand $i_{k-1}$. We can augment $H$ to connect each $t_{i_j}$ to
  $s_{i_{j+1\bmod k}}$, $0\le j\le k-1$ without using any node from
  $\Gamma(r)$, since these nodes are in the same component in
  $G\setminus\Gamma(r)$. But then we have a path $P$ between $s_{i_{k-1}}$ and
  $t_{i_{k-1}}$ and the extension part $P^*$ does not contain any vertex from
  $\Gamma(r)$. This is a contradiction since the arrival threshold for the
  demand $i_{k-1}$ is at least $r$.
\end{proof}


Lemma~\ref{lem:multiwaycut} shows that cutting $\Gamma(r)$ highly disconnects
the demands in $D(r)$. Indeed this implies a bound on the \textit{toughness} of
the graph. Toughness, first defined by Chv{\'a}tal~\cite{C73} and later
generalized by Agrawal \textit{et al.}~\cite{AKR91b}, is a measure of how easy
it is to disconnect a graph into many components by removing a few vertices.
More formally, the toughness of a graph is defined as $\min_{X\subseteq V}
\frac{|X|}{|\CC(G\setminus X)|}$. For the spanning tree variant of the problem,
it is not hard to see that $\OPT$ is at least the reciprocal of toughness.
Although it is more involved, we can still establish a similar relation for the
non-uniform Steiner forest problem (see Lemma~\ref{lem:fitting}). However,
first we need to show a lower bound on the number of demands separated by
$\Gamma(r)$.

%\vlnote{for toughness: although it can be proven directly, we use a dual-fitting analysis (to show that toughness of a cut is a lower bound) mainly because it makes the analysis easier for non-uniform bounds and also to put this approach in perspective with the primal-dual methods designed for online weighted variants of the Steiner connectivity problems.
%	In the analysis, they use the \textit{toughness} of a graph to bound $b^*$, the optimal solution. Toughness, first defined by Chv{\'a}tal~\cite{C73}, is a measure of how easy it is to disconnect a graph into many components by removing a few vertices. More formally, let $\CC(G)$ denote the collection of connected components of a graph $G$. For a subset of vertices $X\subseteq V$, let $G\setminus X$ denote the subgraph obtained from $G$ by removing $X$. The toughness of a graph is defined as $\min_{X\subseteq V} \frac{|X|}{|\CC(G\setminus X)|}$. For the spanning tree variant of the problem, it is not hard to see that $b^*$ is at least the reciprocal of toughness. A similar relation can be shown for the Steiner forest variant by restricting the dominator to the components that separate the demands. Using this to bound $b^*$ together with ideas similar to their work~\cite{AKR91b} in STOC'91, Agrawal \textit{et al.} analyze their algorithm obtained from the reduction to the concurrent flow problem.}


We establish a lower bound for $|D(r)|$ with respect to the load of vertices in
$\Gamma(r)$.
For any $r,b> 0$ we define $\Gamma_b(r):=\{\ell_{\alg}^+(v)\ge r\wedge b_v\ge
b\}$, as the set of nodes with degree bound at least $b$ that have uptick load at least
$r$ in the final online solution. We further define
\begin{equation*}
\operatorname{excess}(r,b)=\sum_{v\in
  \Gamma_b(r)}\!\!\Big(\operatorname{deg}_{\alg}(v)-\lceil r b_v\rceil+2\Big)\enspace,
\end{equation*}
which sums the (absolute) load that nodes in $\Gamma_b(r)$ receive \emph{after}
their \emph{uptick load} became $r$ or larger. The following lemma relates $|D(r)|$ to 
$\operatorname{excess}(r,b)$.
\begin{lemma} \label{lem:largedemand}
For any $r,b>0$, 
%\begin{equation*}
$\operatorname{excess}(r,b)\le 2|D(r)|+3|\Gamma_b(v)|$.
%\end{equation*}
%\frac{\sum_{v\in \Gamma_b(r+\frac{2}{b})} (\ell(v)-r-2/b) b_v}{4} - |\Gamma_b(r+2/b)| \enspace .\]
\end{lemma}
\begin{proof}
  Consider some online step $i$.
  Let $H$ denote the output of the previous step. Let $P^*_i$ be the extension
  part of the path selected by GA and let $V(P^*_i)$ denote the endpoints of
  edges of $P^*_i$. Since in GA we break ties in favor of the path with the
  smaller number of edges, we can assume that the path does not go through a
  connected component of $H$ more than once, i.e., for every $C\in \CC(H)$,
  $|V(P^*_i)\cap C| \leq 2$.

  Consider the variable quantity $\delta(r,b):=\sum_{v: \ell^+_H(v)\geq r
    \wedge b_v\geq b}(\deg_H(v)-\lceil r b_v \rceil+2)$ throughout the steps of GA
  where $H$ denotes the output of the algorithm at every step. Intuitively, at
  each step $\delta(r,b)$ denotes the total increment in degrees of those
  vertices in $\Gamma_b(r)$ that already reached uptick load $r$. In
  particular, at the end of the run of GA,
  $\delta(r,b)=\operatorname{excess}(r,b)$.

  Now suppose at step $i$ adding the edges $P^*_i$ to $H$ increases
  $\delta(r,b)$ by $q_i$. There are two reasons for such an increase. On the
  one hand, if the demand $i$ is from $D(r)$ it may simply increase 
  $\operatorname{deg}_H(v)$ for some node with uptick load at least $r$. On the
  other hand also if the demand is not from $D(r)$ it may cause a node to
  increase its uptick load to $r$ in which case it could contribute to the
  above sum with at most 1 (in a step the degree may increase by 2; the first
  increase by 1 could get the uptick load to $\ge r$ and the second increase
  contributes to the sum). 

  Clearly increases of the second type can accumulate to at most
  $|\Gamma_b(r)|$. In order to derive a bound on the first type of increases
  recall that we assume that endpoints of demands are distinct vertices with
  degree one and thus $s_i$ and $t_i$ are outside any connected component of
  $H$. Since $V(P^*_i)$ contains at most two vertices of a connected component
  of $H$, we can assert that the path selected by GA is passing through at
  least $q_i/2$ components of $H$ that contain some vertices of $\Gamma_b(r)$.
  Hence, after adding $P^*_i$ to the solution, the number of connected
  components of the solution that contain some vertices of $\Gamma_b(r)$
  decreases by at least $(q_i-2)/2$. However, throughout all the steps, the
  total amount of such decrements cannot be more than the number of vertices in
  $\Gamma_b(r)$.
%
%
%  On the
%  other hand, the number of such components may only increase when the uptick
%  load of a vertex increases from below $r$ to at least $r$. Since $b_v\geq b$
%  for every $v\in \Gamma^b(v)$, this may only happen in iterations where the
%  arrival threshold is at least $r-\frac{2}{b}$ (note that the degree of a
%  vertex may increase by at most two after serving a request). Therefore the
%  number of connected components that contain some vertices of $\Gamma_b(r)$
%  increases at most $|D(r-2/b)|$ times (by at most one at each such iteration).
%
%However, throughout all the steps, the total amount of such decrements cannot be more than the number of vertices in $\Gamma(r)$.
Therefore
\begin{align*}
%\sum_{v\in \Gamma_b(r)} \deg_{\alg}(v)-\lceil r b_v \rceil
\operatorname{excess}(r,b)
	&=\sum_{i\in D(r)} q_i+\sum_{i\notin D(r)} q_i\\
	&= 2 |D(r)| + \sum_{i\in D(r)} (q_i-2) +|\Gamma_b(r)|\\
    &\le 2|D(r)| +3|\Gamma_b(r)|\enspace,
\end{align*}
and the lemma follows.
\end{proof}

% \begin{lemma} \label{lem:largedemand}
% For every real value $r> \frac{2}{n-1}$, and $b\in \{1,\ldots, n-1 \}$,
% \[ |D(r)| \geq \frac{\sum_{v\in \Gamma_b(r+\frac{2}{b})} (\ell(v)-r-2/b) b_v}{4} - |\Gamma_b(r+2/b)| \enspace .\]
% \end{lemma}
% \begin{proof}
%   Consider an online step $i$ for which the arrival threshold $\tau_i\geq r$.
%   Let $H$ denote the output of the previous step. Let $P^*_i$ be the extension
%   part of the path selected by GA and let $V(P^*_i)$ denote the endpoints of
%   edges of $P^*_i$. Since in GA we break ties in the favor of the path with the
%   smaller number of edges, we can assume that the path does not go through a
%   connected component of $H$ more than once, i.e., for every $C\in \CC(H)$,
%   $|V(P^*_i)\cap C| \leq 2$.

%   Consider the variable quantity $\delta(r):=\sum_{v: \ell^+_H(v)\geq r \wedge
%     b_v\geq b} \deg_H(v)-\lceil r b_v \rceil$ throughout the steps of GA where
%   $H$ denotes the output of the algorithm at every step. Intuitively, at each
%   step $\delta(r)$ denotes the total increment in degrees of vertices in
%   $\Gamma_b(r)$. In particular, at the end of the run of GA,
%   $\delta(r)=\sum_{v\in \Gamma_b(r)} \deg_{\alg}(v)-\lceil r b_v \rceil$. Now
%   suppose at step $i$ adding the edges $P^*_i$ to $H$ increments $\delta(r)$ by
%   $q_i$. Recall that we assume the endpoints of demands are distinct vertices
%   with degree one and thus $s_i$ and $t_i$ are outside any connected component
%   of $H$. On the other hand, since $V(P^*_i)$ contains at most two vertices of
%   a connected component of $H$, we can assert that the path selected by GA is
%   passing through at least $q_i/2$ components of $H$ that contain some vertices
%   of $\Gamma_b(r)$. Hence, after adding $P^*_i$ to the solution, the number of
%   connected components of the solution that contain some vertices of
%   $\Gamma_b(r)$ decreases by at least $(q_i-2)/2$. On the other hand, the
%   number of such components may only increase when the uptick load of a vertex
%   increases from below $r$ to at least $r$. Since $b_v\geq b$ for every $v\in
%   \Gamma_b(v)$, this may only happen in iterations where the arrival threshold
%   is at least $r-\frac{2}{b}$ (note that the degree of a vertex may increase by
%   at most two after serving a request). Therefore the number of connected
%   components that contain some vertices of $\Gamma_b(r)$ increases at most
%   $|D(r-2/b)|$ times (by at most one at each such iteration).

% %However, throughout all the steps, the total amount of such decrements cannot be more than the number of vertices in $\Gamma(r)$.
% Therefore we have:
% \begin{align*}
% \sum_{v\in \Gamma_b(r)} \deg_{\alg}(v)-\lceil r b_v \rceil
% 	&=\sum_i q_i\\
% 	&=\sum_{i\in D(r-2/b)} q_i & q_i>0 \Longrightarrow \tau_i\geq r-2/b\\
% 	&= 2 |D(r-2/b)| + \sum_{i\in D(r-2/b)} (q_i-2) \\
% 	&\leq 2 |D(r-2/b)| + 2 |D(r-2/b)| \\
% 	&= 4 |D(r-2/b)|
% \end{align*}
% This proves the lemma since
% \[ \sum_{v\in \Gamma_b(r)} \deg_{\alg}(v)-\lceil r b_v \rceil \geq \sum_{v\in \Gamma_b(r)} (\ell(v)-r) b_v - |\Gamma_b(r)| \enspace . \]
%\end{proof}

Let $\Delta>0$ denote the minimum degree bound of a vertex with non-zero degree in
an optimal solution. Note that this definition implies that $\OPT\ge1/\Delta$. For a set of vertices $\Gamma$, let $b(\Gamma)=\sum_{v\in \Gamma} b_v$.
We now describe the main dual-fitting argument for
bounding the maximum load in \alg{}. 

\begin{lemma} \label{lem:fitting}
	For any $r>0$, ${|D(r)|}/{b(\Gamma_{\Delta}(r))}\leq \OPT$.
\end{lemma}
\begin{proof}
  Let $G_{\Delta}$ denote the graph obtained from $G$ by removing vertices with
  degree bound below $\Delta$. Similarly, let $\Mc{S}_{\Delta}$ denote the
  collection of sets that separate a demand in $G_{\Delta}$. Consider a
  slightly modified dual program $\text{\ref{LP:dualsf}}_{\Delta}$ defined on
  $G_{\Delta}$ and $\Mc{S}_{\Delta}$, i.e., we obtain
  $\text{\ref{LP:dualsf}}_{\Delta}$ from the original dual program by removing
  all vertices with degree bound below $\Delta$. We note that the objective
  value of a dual feasible solution for $\text{\ref{LP:dualsf}}_{\Delta}$ is
  still a lower bound for $\OPT$. In the remainder of the proof, we may refer
  to $\text{\ref{LP:dualsf}}_{\Delta}$ as the dual program.
%
  Recall that in a feasible dual solution, we need to define a dual value
  $\y(S)$ for every cut $S\in \Mc{S}_{\Delta}$ such that for every edge
  $e=(u,v)$ the total value of cuts that contain $e$ does not exceed
  $\z(u)+\z(v)$. On the other hand, $\sum_v \z(v) b_v$ cannot be more than one.

  For a
  real value $r> 0$, we construct a dual vector $(\y_r,\z_r)$ as follows.
  For every $v\in \Gamma_{\Delta}(r)$, set
  $\z_r(v)={1}/{b(\Gamma_{\Delta}(r))}$; for other vertices set
  $\z_r(v)=0$. For every component $S\in \CC(G_{\Delta}\setminus
  \Gamma_{\Delta}(r)) \cap \Mc{S}_{\Delta}$, set
  $\y_r(S)={1}/{b(\Gamma_{\Delta}(r))}$; for all other sets set
  $\y_r(S)=0$. We prove the lemma by showing the feasibility of the dual vector
  $(\y_r,\z_r)$ for $\text{\ref{LP:dualsf}}_{\Delta}$.


  Consider an arbitrary component $C\in \CC(G\setminus \Gamma(r))$. By
  definition, $C$ separates at least one demand. Let $i$ be such a demand and
  let $t_i\in C$ denote an endpoint of it. Removing vertices with degree bound
  below $1/\Delta$ from $C$ may break $C$ into multiple smaller components.
  However, an endpoint of a demand has degree bound infinity, and, hence, the
  component that contains $t_i$ belongs to $\Mc{S}_\Delta$. Therefore
  $|\CC(G\setminus \Gamma(r)) \cap \Mc{S}|\leq |\CC(G_{\Delta}\setminus
  \Gamma_{\Delta}(r)) \cap \Mc{S}_{\Delta}|$; which by
  Lemma~\ref{lem:multiwaycut} leads to $|\CC(G_{\Delta}\setminus
  \Gamma_{\Delta}(r)) \cap \Mc{S}_{\Delta}| \geq |D(r)|+1$. Therefore the dual
  objective for the vector $(\y_r,\z_r)$ is at least

  \[ \sum_{S\in \Mc{S}_{\Delta}} \y_r(S) = \sum_{S\in \CC(G_{\Delta}\setminus
    \Gamma_{\Delta}(r)) \cap \Mc{S}_{\Delta}} \frac{1}{b(\Gamma_{\Delta}(r))}
  \geq \frac{|D(r)|+1}{b(\Gamma_{\Delta}(r))} \enspace .\]
  Thus we only need to show that $(\y_r,\z_r)$ is feasible for
  Program~$\text{\ref{LP:dualsf}}_{\Delta}$. First, by construction we have
  \[ \sum_v \z_r(v) b_v = \sum_{v\in \Gamma_{\Delta}(r)}
  \frac{1}{b(\Gamma_{\Delta}(r))} \cdot b_v =1 \enspace . \]
  Now consider an arbitrary edge $e=(u,v)$. If $e$ does not cross any of the
  components in $\CC(G_{\Delta}\setminus \Gamma_{\Delta}(r))$, then $\sum_{S:
    e\in \delta(S)} \y_r(S)=0$ and we are done. Otherwise, $\sum_{S: e\in
    \delta(S)} \y_r(S)={1}/{b(\Gamma_{\Delta}(r))}$. However, exactly one
  endpoint of $e$ is in $\Gamma_{\Delta}(r)$. Thus
  $\z_r(u)+\z_r(v)={1}/{b(\Gamma_{\Delta}(r))}$, which implies that the
  dual vector is feasible.
\end{proof}


\noindent
We now have all the ingredients to prove the main theorem.
\smallskip

\begin{proof}[of Theorem~\ref{thm:mainlog}]
  Let \alg{} denote the final output of the greedy algorithm. Let $h$ denote
  the maximum load of a vertex in $\alg$, i.e., $h=\max_v \ell_{\alg}(v)$.
  Furthermore, let $h_{\Delta}=\max_{v: b_v\geq \Delta} \ell_{\alg}(v)$. 
In the following we first show that $h_{\Delta}\le O(\log n)\cdot\OPT$.
For this we use the folowing claim.

%In
%  what follows, we show that there always exists an $r> 1/\Delta$ for which
%  $\frac{|D(r)|}{b(\Gamma_{\Delta}(r))}\geq \frac{h_{\Delta}}{O(\lg(n))}$,
%  which by Lemma~\ref{lem:fitting} implies that $h_{\Delta}\leq O(\lg n) \OPT$.




\begin{claim}
There exists an $r>0$ such that 
\begin{equation*}
\operatorname{excess}(r,\Delta)\ge
\frac{h_\Delta-1/\Delta}{4\log_2n+6}\cdot b(\Gamma_\Delta(r))-|\Gamma_\Delta(r)|\enspace.
\end{equation*}
\end{claim}
\begin{proof}
  Recall that $\Gamma_{\Delta}(r)$ is the set of vertices with uptick load at
  least $r$ in \alg{} and degree bound at least $\Delta$.
  The function $b(\Gamma_\Delta(r))$ is non-increasing with $r$ since for every
  $r_1<r_2$, $\Gamma_{\Delta}(r_2)\subseteq \Gamma_{\Delta}(r_1)$. For
  $r=1/\Delta$, $b(\Gamma_\Delta(r))\le n(n+1)\Delta$ as a node with  degree bound
  $b_v> (n+1)\Delta$ will have uptick load at most $(n+1)/b_v<{1}/{\Delta}$,
  and, hence, will not be in $\Gamma_\Delta(r)$.
  Also, $r<h_\Delta$ implies that $b(\Gamma_\Delta(r))\ge\Delta$ as there
  exists a node with load $h_\Delta$ in $\Gamma_\Delta(r)$ and this node has
  degree bound at least $\Delta$.

  We now partition the range of $r$ (from $1/\Delta$ to $h_\Delta$) into
  logarithmically many intervals. We define the $q$-th interval by
\begin{align*}
U(q) &= \left\{ r\mid {1}/{\Delta} 
\le r < h_{\Delta} \ \wedge \ 2^q/\Delta \leq b(\Gamma_{\Delta}(r)) <
2^{q+1}/\Delta \right\} \enspace,
\end{align*}
for $q\in\{0,\dots,\lceil\log_2((n+1)n)\rceil\}$.
We further set
%\begin{align*}
$\overline{r}(q) = \max U(q)$ and $\underline{r}(q) = \min U(q)$,
%\end{align*}
and call $\overline{r}(q)-\underline{r}(q)$ the length of the $q$-th interval.
Since there are only $2\log_2n+3$ possible choices for $q$ there must exist an
interval of length at least $(h_\Delta-1/\Delta)/(2\log_2n+3)$.

Consider a node $v$ that is contained in $\Gamma_\Delta(\overline{r})$
and, hence, also in $\Gamma_\Delta(\underline{r})$. This node starts
contributing to $\operatorname{excess}(\underline{r},\Delta)$, once its uptick
load reached $\underline{r}$ and contributes at least until its uptick load
reaches $\overline{r}$. Hence, the total contribution is at least
$\operatorname{deg}(\overline{r})-\operatorname{deg}(\underline{r})$, where
$\operatorname{deg}(\overline{r})$ and $\operatorname{deg}(\underline{r})$
denotes the degree of node $v$ when reaching uptick load $\overline{r}$ and
$\underline{r}$, respectively. We have,
\begin{equation*}
\begin{split}
\operatorname{deg}(\overline{r})-\operatorname{deg}(\underline{r})
&= (\lceil\overline{r}b_v\rceil-2)-(\lceil\underline{r}b_v\rceil-2)\\
&\ge (\overline{r}-\underline{r})b_v-1\enspace.
\end{split}
\end{equation*}
Summing this over all nodes in $\Gamma_\Delta(\overline{r})$ 
gives 
\begin{equation*}
\begin{split}
\operatorname{excess}(\underline{r},\Delta) 
  &\ge (\overline{r}-\underline{r})\cdot b(\Gamma_\Delta(\overline{r}))-|\Gamma_\Delta(\overline{r})|\\
  &\ge \frac{1}{2}(\overline{r}-\underline{r})\cdot b(\Gamma_\Delta(\underline{r}))-|\Gamma_\Delta(\underline{r})|\\
  &\ge \frac{h_\Delta-1/\Delta}{4\log_2n+6}\cdot b(\Gamma_\Delta(\underline{r}))-|\Gamma_\Delta(\underline{r})|\enspace,
\end{split}
\end{equation*}
where the second inequality uses the fact that
$|\Gamma_\Delta(\overline{r})|\le|\Gamma_\Delta(\underline{r})|\le|\Gamma_\Delta(\overline{r})|/2$.
\end{proof} % claim


\begin{claim}
$h_{\Delta}\leq (24\log_2 n+37) \OPT$.
\end{claim}
\begin{proof}
If we use the $r$ from the previous claim and solve for $h_\Delta$ we obtain
\begin{equation*}
\begin{split}
h_\Delta
&\le(4\log_2 n+6)\cdot\frac{\operatorname{excess}(r,\Delta)+\Gamma_\Delta(r)}{b(\Gamma_\Delta(r))}+\frac{1}{\Delta}\\
&\le(4\log_2 n+6)\cdot\frac{2D(r)+4\Gamma_\Delta(r)}{b(\Gamma_\Delta(r))}+\frac{1}{\Delta}\\
&\le(4\log_2 n+6)\cdot \Big(2\OPT+4\frac{1}{\Delta}\Big)+\frac{1}{\Delta}\\
&\le(24\log_2 n+37)\cdot \OPT\enspace.
\end{split}
\end{equation*}
Here the second inequality is due to Lemma~\ref{lem:largedemand}, the third
uses Lemma~\ref{lem:fitting} and the fact that
$b(\Gamma_\Delta(r))\ge\Delta|\Gamma_\Delta(r)|$. The last inequality uses $\OPT\ge 1/\Delta$.
\end{proof}

\medskip
\noindent
We now bound the maximum load $h$ in terms of the restricted maximum load $h_{\Delta}$.
Consider a vertex $v^*$ with maximum load $\ell_{\alg}(v^*)=h$. If $b_{v^*}\geq
\Delta$ then $h_{\Delta}=h$ and we are done. Otherwise consider the last
iteration $i$ in which the degree of $v^*$ is increased in the solution. Let
$H$ denote the output of the algorithm at the end of the previous iteration $i-1$. The
degree of $v^*$ in the online solution is increased by at most two at iteration
$i$. Hence
\[h	\leq \ell^+_H(v^*) \leq \tau_i  \enspace .\]
Recall that in our greedy algorithm, $\tau_i$ is the minimum uptick load of a
path that satisfies the new demand. Let $P$ denote a path that connects $s_i$
and $t_i$ in an optimal solution. Recall that by the definition, $b_v\geq
\Delta$ for every vertex $v$ of $P$. For every vertex $v$ in $P$ we have
\begin{align*}
\tau_i &\leq \ell^+_H(v) \\
	&\leq h_{\Delta}+\frac{2}{b_v} &\ell_H(v)\leq \ell_{\alg}(v)\leq h_{\Delta}\\
	&\leq h_{\Delta}+\frac{2}{\Delta} & b_v\geq \Delta\\
	&\leq h_{\Delta}+2\OPT	 & \OPT\geq 1/\Delta\\
	&\leq O(\log n)\cdot\OPT &\text{by the above claim}
\end{align*}
Therefore leading to $h \leq O(\log n)\cdot\OPT$.
\end{proof}

% \begin{theorem}
%   There exists an online algorithm such that the maximum load of a vertex in
%   the final output is at most $(28\lg n +16)\OPT$.
% \end{theorem}
% \begin{proof}
%   Let \alg{} denote the final output of the greedy algorithm. Let $h$ denote
%   the maximum load of a vertex in $\alg$, i.e., $h=\max_v \ell_{\alg}(v)$.
%   Furthermore, let $h_{\Delta}=\max_{v: b_v\geq \Delta} \ell_{\alg}(v)$. In
%   what follows, we show that there always exists an $r> 1/\Delta$ for which
%   $\frac{|D(r)|}{b(\Gamma_{\Delta}(r))}\geq \frac{h_{\Delta}}{O(\lg(n))}$,
%   which by Lemma~\ref{lem:fitting} implies that $h_{\Delta}\leq O(\lg n) \OPT$.

% \begin{claim}
% $h_{\Delta}\leq (28\lg n+14) \OPT$.
% \end{claim}
% \begin{proof}
%   We note that $\OPT\geq 1/\Delta$. Thus we focus only on instances where
%   $h_{\Delta}\geq \frac{4\lg n+3}{\Delta}$, otherwise the claim is trivial.
%   Recall that $\Gamma_{\Delta}(r)$ is the set of vertices with uptick load at
%   least $r$ in \alg{} and degree bound at least $\Delta$. We know that the
%   function $b(\Gamma_{\Delta}(r))$ is non-increasing in $r$ since for every
%   $r_1<r_2$, $\Gamma_{\Delta}(r_2)\subseteq \Gamma_{\Delta}(r_1)$. Recall that
%   for every vertex $v$, $b_v\in \{1,\dots, n-1\}$ and thus the total $b(V)<
%   n^2$. Now for every integer $q\in \{0,\ldots, \lfloor \lg(n^2) \rfloor \}$,
%   define
% \begin{align*}
% U(q) &= \left\{ r | \max\{\frac{2}{n-1}, \frac{1}{\Delta}\} < r < h_{\Delta} \ \wedge \ 2^q \leq b(\Gamma_{\Delta}(r)) < 2^{q+1} \right\} \enspace ;\\
% \overline{r}(q) &= \max U(q) \enspace ;\\
% \underline{r}(q) &= \min U(q) \enspace .\\
% \end{align*}
% We again emphasize that since $b(.)$ is monotone, $U(q)$ contains all the real values between $\underline{r}(q)$ and $\overline{r}(q)$. Now let 
% \begin{align*}
% q^* &=\argmax_q \{\overline{r}(q)-\underline{r}(q)\} \enspace .
% \end{align*}
% Observe that the range of $r$ is from $1/\Delta$ to $h_{\Delta}$. Therefore
% $\overline{r}(q^*)-\underline{r}(q^*)\geq
% \frac{h_{\Delta}-1/\Delta}{2\lg(n)+1}$ since we have at most $1+2\lg n$
% different possible values for $q$. Furthermore, note that we have assumed at
% the beginning that $h_{\Delta}\geq \frac{4\lg n+3}{\Delta}$. Thus
% $\overline{r}(q^*)-\underline{r}(q^*)\geq 2/\Delta$.

% We claim that the desired ratio of Lemma~\ref{lem:fitting} is achieved for $\underline{r}(q^*)$. For simplicity, in what follows we drop the term $q^*$ when it is clear from the context. We have
% \begin{align*}
% 4|D(\underline{r})|
% 	&\geq \sum_{v\in \Gamma_{\Delta}(\underline{r}+2/\Delta)} (\ell(v)-\underline{r}-2/\Delta) b_v
% 	- |\Gamma_{\Delta}(\underline{r}+2/\Delta)|  & \text{by Lemma~\ref{lem:largedemand}}\\
% 	&\geq \sum_{v\in \Gamma_{\Delta}(\overline{r})} (\ell(v)-\underline{r}-2/\Delta) b_v
% 	- |\Gamma_{\Delta}(\underline{r}+2/\Delta)| & \overline{r}\geq \underline{r}+ 2/\Delta \\
% 	&\geq \sum_{v\in \Gamma_{\Delta}(\overline{r})} (\overline{r}-2/b_v-\underline{r}-2/\Delta) b_v 
% 	- |\Gamma_{\Delta}(\underline{r}+2/\Delta)| & v\in \Gamma_{\Delta}(\overline{r}) \Rightarrow \ell(v)\geq \overline{r}-2/b_v \\
% 	&\geq (\overline{r}-\underline{r}-4/\Delta) b(\Gamma_{\Delta}(\overline{r})) 
% 	- |\Gamma_{\Delta}(\underline{r}+2/\Delta)| & b_v\geq \Delta\text{ for }v\in \Gamma_{\Delta}(r)\\
% 	&\geq (\overline{r}-\underline{r}-4/\Delta) 2^{q^*}
% 	- |\Gamma_{\Delta}(\underline{r}+2/\Delta)| & \overline{r}\in U(q^*)\\
% 	&\geq (\overline{r}-\underline{r}-4/\Delta) 2^{q^*}
% 	- |\Gamma_{\Delta}(\underline{r})| \enspace .
% \end{align*}
% Finally to use Lemma~\ref{lem:fitting}, we show that
% \begin{align*}
% \frac{D(\underline{r})}{b(\Gamma_{\Delta}(\underline{r}))}
% 	&\geq \frac{(\overline{r}-\underline{r}-4/\Delta) 2^{q^*} - |\Gamma_{\Delta}(\underline{r})|}{4 b(\Gamma_{\Delta}(\underline{r}))} \\
% 	&\geq \frac{(\overline{r}-\underline{r}-4/\Delta) 2^{q^*}}{4\cdot 2^{q^*+1}} - \frac{|\Gamma_{\Delta}(\underline{r})|}{4b(\Gamma_{\Delta}(\underline{r}))} & \underline{r}\in U(q^*)\\
% 	&\geq \frac{\overline{r}-\underline{r}-4/\Delta}{8} - \frac{1}{4\Delta} & b_v\geq \Delta \text{ for } v\in \Gamma_{\Delta}(r)\\
% 	&\geq \frac{h_{\Delta}}{8(1+2\lg(n))}-\frac{1}{2\Delta} - \frac{1}{4\Delta} \enspace .
% \end{align*}
% which completes the proof since $\OPT\geq \frac{1}{\Delta}$.
% \end{proof}

% We now bound the maximum load $h$ by the restricted maximum load $h_{\Delta}$.
% Consider a vertex $v^*$ with maximum load $\ell_{\alg}(v^*)=h$. If $b_{v^*}\geq
% \Delta$ then $h_{\Delta}=h$ and we are done. Otherwise consider the last
% iteration $i$ in which the degree of $v^*$ is increased in the solution. Let
% $H$ denote the output of the algorithm after the previous iteration $i-1$. The
% degree of $v^*$ in the online solution is increased by at most two at iteration
% $i$. Hence
% \[h	\leq \ell^+_H(v^*) \leq \tau_i  \enspace .\]

% Recall that in our greedy algorithm, $\tau_i$ is the minimum uptick load of a
% path that satisfies the new demand. Let $P$ denote a path that connects $s_i$
% and $t_i$ in an optimal solution. Recall that by the definition, $b_v\geq
% \Delta$ for every vertex $v$ of $P$. For every vertex $v$ in $P$ we have
% \begin{align*}
% \tau_i &\leq \ell^+_H(v) \\
% 	&\leq h_{\Delta}+\frac{2}{b_v} &\ell_H(v)\leq \ell_{\alg}(v)\leq h_{\Delta}\\
% 	&\leq h_{\Delta}+\frac{2}{\Delta} & b_v\geq \Delta\\
% 	&\leq h_{\Delta}+2\OPT	& \OPT\geq 1/\Delta\\
% 	&\leq O(\lg n) \OPT	&\text{by the above claim}
% \end{align*}
% Therefore leading to $h \leq O(\lg n) \OPT$
%\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "notes"
%%% End: 

==> draft (1)/dblower.tex <==

\def\mydeg{\operatorname{deg}}
\def\mydegb{\operatorname{deg}'}

\section{An Asymptotically Tight Lower Bound}
In the following we show a lower bound for 
\odbst{}.
Consider a  graph $G=(X \uplus Z, E)$, with $|Z|=2^\ell$ and
$|X|=\binom{2^\ell}{2}$. 
For every pair $\{z_1,z_2\}$ of nodes from $Z$ there exists 
an edge $\{z_1,z_2\}\in E$ and a node $x\in X$ that is connected
to $z_1$ and $z_2$. An arbitrary node from $Z$ acts as root for the  Steiner
tree problem.

For a node $z\in Z$, an algorithm $A$, and a request sequence $\sigma$
(consisting of nodes from $X$) we use $\mydeg_{A,\sigma}(z)$ to denote the
number of neighbors of $z$ \emph{among all nodes from X} in the Steiner tree
obtained when running algorithm $A$ on request sequence $\sigma$. Similarly, we
use $\mydegb_{A,\sigma}(z)$ to denote the number of those neighbors of $z$ that
also appear in $\sigma$. Note that $\mydeg(\cdot)$ and $\mydegb(\cdot)$ ignore
edges between nodes from $Z$ as an algorithm (online or offline) can simply
connect all nodes in $Z$ in a cycle which increases the degree of any node by
only 2.


\def\ex{\operatorname{E}}
\begin{lemma} Fix a possibly randomized online algorithm $A$.
For any subset $S\subseteq Z$, $|S|=2^s$, $0\le s\le \ell$ there exists a request sequence
$\sigma_S$ consisting of terminals from $X$ s.t.\
\begin{itemize}
\item for a node $x\in \sigma_S$ both its neighbors in $G$ are from set $S$;
\item there exists a node $z^*\in S$ with $\ex[\mydegb_{A,\sigma}(z^*)]\ge s/2$;
\item there exists an offline algorithm $\mathrm{OFF}$ for servicing requests
  in $\sigma$ with 
  $\max_{z\in
    S}\{\mydeg_{\mathrm{OFF},\sigma}(z)\}\le 1$, and
  $\mydeg_{\mathrm{OFF},\sigma}(z)=0$ for $z\in (Z\setminus S)\cup \{z^*\}$.
\end{itemize}
\end{lemma}
\begin{proof}
We prove the lemma by induction over $s$. The base case $s=0$ holds trivially
when choosing the empty request sequence. For the induction step consider an
arbitrary subset $S\subseteq Z$ with $|S|=2^{s+1}$. Partition $S$ into two
disjoint subsets $S_1$ and $S_2$ of cardinality $2^{s}$ each.

Let $\sigma_1$ be the request sequence that exists due to induction hypothesis
for set $S_1$. Hence, there is a node $z_1^*\in S_1$ with
$\ex[\mydeg'_{A,\sigma_1}(z_1^*)]\ge s/2$. Now, let $\tilde{A}$ behave like algorithm $A$
\emph{after} it already received a request sequence $\sigma_1$ (hence, it
starts with all edges that are chosen when running $A$ on $\sigma_1$;
note, however, that $\mydegb_{\tilde{A},\sigma_2}(\cdot)$ only takes into
account edges incident to nodes from $\sigma_2$). Due to
induction hypothesis for $\tilde{A}$ and set $S_2$ there exists a request sequence
$\sigma_2$ such that $\ex[\mydegb_{\tilde{A},\sigma_2}(z_2^*)]\ge s/2$ for a node $z_2^*\in
S_2$. Hence, the request sequence $\sigma=\sigma_1\circ\sigma_2$ fulfills
$\ex[\mydegb_{A,\sigma}(z_1^*)]\ge s/2$ and $\ex[\mydegb_{A,\sigma}(z_2^*)]\ge s/2$.

We extend the request sequence by appending the node $x$ that is connected to
$z_1^*$ and $z_2^*$ in $G$. After serving the request one of the edges
$\{x,z_1\}$ or $\{x,z_2\}$ must be chosen with probability at least 1/2 by $A$.
Hence, afterwards either $\ex[\mydegb_{A,\sigma}(z_1^*)]$ or
$\ex[\mydegb{\delta}_{A,\sigma}(z_2^*)]$ must be at least $(s+1)/2$.

It remains to argue that there exists a good offline algorithm. Combining the
offline algorithms $\mathrm{OFF}_1$ and $\mathrm{OFF}_2$ for $\sigma_1$ and
$\sigma_2$ gives an offline algorithm for $\sigma_1\circ\sigma_2$ that 
has $\max_{z}\{
\mydeg_{\mathrm{OFF},\sigma_1\circ\sigma_2}(z)\}\le 1$ 
and $\mydeg_{\mathrm{OFF},\sigma_1\circ\sigma_2}(z)\}=0$ for $z\notin S_1\cup
S_2$ and for $z\in\{z_1^*,z_2^*\}$. Now, when the node $x$ connected to $z_1^*$
and $z_2^*$ is appended to the request sequence the offline algorithm can
serve this request by either buying edge $\{x,z_1\}$ or $\{x,z_2\}$, and can
therefore gurantee that $z_*$ (either $z_1$ or $z_2$) has degree $0$.
\end{proof}

\medskip
\noindent
\begin{proof}[of Theorem~\ref{thm:LBst}]
	Choosing $s=\log n$ in the above lemma gives our lower bound.
\end{proof}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "notes"
%%% End: 

==> draft (1)/figures.tex <==
\section{Figures}

\begin{algorithm}[!h]
	\textbf{Input:} A graph $G$, and an online stream of demands $(s_1,t_1), (s_2,t_2), \ldots$.
	
	\textbf{Output:} A set $H$ of edges such that every given demand $(s_i,t_i)$ is connected via $H$.
	
	\textbf{Offline Process:}
		\begin{algorithmic}[1]
			\STATE Initialize $H=\varnothing$.
		\end{algorithmic}
	
	\textbf{Online Scheme; assuming a demand $(s_i,t_i)$ is arrived:}
	
	\begin{algorithmic}[1]
		\STATE Compute $P_i$, a $(s_i, t_i)$-path with the smallest uptick load $\ell^+_H(P_i^*)$ in its extension part.
		\begin{itemize}
			\item Shortcut the connected components of $H$ by replacing the edges of a component with that of a clique.
			\item In the resulting graph, define the distance of a vertex $v$ from $s_i$ as the minimum uptick load of a $(s_i,v)$-path.
			\item Find $P_i$ by evoking a Dijkstra-like algorithm according to this notion of distance. 
		\end{itemize}
		\STATE Set $H=H\cup P_i^*$.
	\end{algorithmic}
	\caption{Online Degree-Bounded Steiner Forest}
	\label{alg:dbsf}
\end{algorithm}

\begin{figure}[!h]
	\begin{center}
		\includegraphics[width=0.7\textwidth]{lemSep.pdf}
	\end{center}
	\caption{Existence of a cycle implies that of a path with low uptick load in its extension part.}
	\label{fig:lemsep}
\end{figure}

==> draft (1)/groupsteiner.tex <==
\subsection{{\sc Online Degree-Bounded Group Steiner Tree}}
%The following describes the first part of Theorem 1.3.
In this section, presenting an adversary scenario, we show there is no deterministic algorithm for \odbgst{} with competitive ratio $o(n)$ even if $G$ is a star graph.

\begin{proof}[of Theorem~\ref{thm:gstLB}]
	For any integer $n>1$, we provide a graph instance $G$ of size $n$ and an online scenario, in which no deterministic algorithm can obtain a competitive ratio better than $n-1$.
	Let $G$ be a star with $n-1$ leaves $v_2$ to $v_{n}$, and $v_{1}$ be the internal node. For an algorithm $\mathcal{A}$, we describe the adversary scenario as follows.
	
	Let $v_{1}$ be the root. Let the first demand group be the set of all leaves. Whenever $\mathcal{A}$ connects a node $v_i$ to $v_1$ in $H$, adversary removes the selected nodes $v_i$ from the next demand groups, until all leaves are connected to $v_1$ in $H$. In particular let $C$ denote the set of all nodes connected to $v_1$ in $H$ so far. Let the demand group be the set of all leaves in $\{v_2, v_3, \ldots, v_n\} \setminus C$. We do this until $\{v_2, v_3, \ldots, v_n\} \setminus C = \emptyset$, which means every leaf is connected to $v_1$ in $H$. $G$ is a star, thus a leaf $v_i$ is connected to $v_1$ in $H$ \text{iff} $H$ includes the edge between $v_i$ and $v_1$. Thus after all demands $\mathcal{A}$ has added all edges in $G$ to $H$. Hence $deg(v_1)=n-1$.
	
	%the group request $g_k$ at step $k$, $R_k$ be $V \setminus C_{k-1}$, where $C_{k-1}$ is the set of nodes that $\mathcal{A}$ has chosen by step $k$. Thus the algorithm has to choose a new node to connect the group. Therefore at each step we are choosing a new node. There are $n$ steps until we request a single node, thus $C_{n}=n$ and the degree for the internal node is $n$.
	Now consider the optimal offline algorithm. Let $g_i$ denote the $i$-th demand group. Assume we have $k$ demand groups. By construction of the demand groups $g_{k} \subset g_{k-1} \subset \ldots \subset g_{1}$. Thus there is a single node that exists in all group demands. Hence the optimal offline algorithms only needs to connect that node to the root in $H$. Therefore, the degree of each node is at most $1$ and the competitive ratio is $n-1$.
\end{proof}


==> draft (1)/intro.tex <==
\section{Introduction}
The problem of satisfying connectivity demands on a graph while respecting
given constraints has been a pillar of the area of network design since the early
seventies~\cite{C73,CGM80,CG82,PY82}. The problem of \dbsp{}, introduced in
Garey and Johnson's \textit{Black Book} of NP-Completeness~\cite{GJ79}, was
first investigated in the pioneering work of F{\"u}rer and
Raghavachari~\cite{FR90} (Allerton'90). In the \dbsp{} problem, the goal is to
construct a spanning tree for a graph $G=(V,E)$ with $n$ vertices whose maximal
degree is the smallest among all spanning trees. Let $b^*$ denote the maximal
degree of an optimal spanning tree. F{\"u}rer and Raghavachari~\cite{FR90}
give a parallel approximation algorithm which produces a spanning tree of
degree at most $O(\log(n) b^*)$.

%\hrnote{This paragraph should be reworded; }
%\hrnote{I reworded the following paragraph; I am still not too happy with it.
%  Right now it means that Agrawal et al. did *only* consider DBST but their
%  algorithm also works for DBSF. Is this correct?}

Agrawal, Klein, and Ravi~(\cite{AKR91a}) consider the following generalizations
of the problem. In the \dbst{} problem we are only required to connect a given
subset $T\subseteq V$. In the even more general \dbsf{} problem the demands
consist of vertex pairs, and the goal is to output a subgraph in which for
every demand there is a path connecting the pair. They design an algorithm
that obtains a multiplicative approximation factor of $O(\log(n))$.
Their main technique is to reduce the problem to
minimizing congestion under integral concurrent flow restrictions and to then
use the randomized rounding approach due to Raghavan and Thompson~(\cite{RT85},
STOC'85).

%a more general variant of the problem, \dbst{}, in which we are only required
%to connect a given set of vertices $T\subseteq V$. They design an algorithm
%that obtains a multiplicative approximation factor of $O(\log(n))$. In fact,
%their algorithm obtains the same guarantee also for \dbsf{}. In this even more
%general variant the demands consist of vertex pairs, and the goal is to output
%a subgraph in which for every demand there is a path connecting the pair.
% 
% 
%%
%%Their algorithm gives the same guarantee
%%for the more general \textit{Steiner forest}\footnote{Also known as generalized
%%  Steiner tree.} variant of the problem. 
%%In \dbsf{}, given a set of demands
%%each in the form of a pair of vertices, 
% 
% 
%Their main technique is to reduce the problem to
%minimizing congestion under integral concurrent flow restrictions and to then
%use the randomized rounding approach due to Raghavan and Thompson~(\cite{RT85},
%STOC'85).

%Agrawal \textit{et
%  al.} use the randomized rounding algorithm of Raghavan and
%Thompson~(\cite{RT85}, STOC'85) in designing their algorithm by reducing the
%problem to minimizing congestion under integral concurrent flow restrictions.

Shortly after the work of Agrawal~\textit{et al.}, in an independent work in
SODA'92 and later J.~of Algorithms'94, F{\"u}rer and
Raghavachari~\cite{FR94} significantly improved the result for \dbsf{} by
presenting an algorithm which produces a Steiner forest with maximum degree at
most $b^*+1$. They show that the same guarantee carries over to the
\textit{directed} variant of the problem as well. Their result is based on
reducing the problem to that of computing a sequence of maximal matchings on
certain auxiliary graphs. This result settles the approximability of the
problem, as computing an optimal solution is NP-hard even in the spanning tree
case.

In this paper, we initiate the study of degree-bounded network design problems
\textit{in an online setting}, where connectivity demands appear over time and must be
immediately satisfied. We first design a deterministic algorithm for \odbsf{}
with a logarithmic competitive ratio. Then we show that this competitive ratio
is asymptotically best possible by proving a matching lower bound for
randomized algorithms that already holds for the Steiner tree variant of the problem.


%We prove several lower bounds for different
%variants of the problem, in particular, we show that the competitive ratio of
%our algorithm is almost tight even for the Steiner tree variant of the problem,
%and even if we are allowed to use randomization.

In the offline scenario, the results of F{\"u}rer,
Raghavachari~\cite{FR90,FR94} and Agrawal, Klein, Ravi~\cite{AKR91a} were the
starting point of a very popular line of work on various degree-bounded network
design problems~\cite{MRSR98,G06,N12,LS13,KKN13,EV14}. We refer the reader to
the next sections for a brief summary. One particular variant that has been
extensively studied is the \textit{edge-weighted} \dbsp{}. Initiated by
Ravi~\textit{et al.} (\cite{MRSR98}, J.~of Algorithms'98), in this version, we
are given a weight function over the edges and a bound $b$ on the maximum
degree of a vertex. The goal is to find a minimum-weight spanning tree with
maximum degree at most $b$. The groundbreaking results obtained by
Goemans~(\cite{G06}, FOCS'06) and Singh and Lau~(\cite{LS07},~STOC'07) settle
the problem by giving an algorithm that computes a minimum-weight spanning tree
with degree at most $b+1$. Slightly worse result are obtained by Singh and
Lau~(\cite{LS13}, STOC'08) for the Steiner tree variant.
Unfortunately, in the online setting it is not possible to obtain a comparable
result. We show that for any (randomized) algorithm $\Mc{A}$ there exists a request
sequence such that $\Mc{A}$ outputs a sub-graph that either has weight
$\Omega(n)\cdot\mathrm{OPT}_b$ or maximum degree $\Omega(n)\cdot b$.


%We show that for any (randomized)
%algorithm $A$ there exists a request sequence that can be handled by an optimum
%algorithm with maximum degree $\mathrm{OPT}_{\mathrm{deg}}$ and weight
%$\mathrm{OPT}_{\mathrm{W}}$, while $A$ either has
%$\ex{\operatorname{deg}}\ge\Omega(n)\cdot\mathrm{OPT}_{\mathrm{deg}}$
%or $\ex{\operatorname{weight}}\ge\Omega(n)\cdot\mathrm{OPT}_{\mathrm{W}}$.
% 
%\hrnote{I think it is very important to mention our lower bound here. Maybe not
%that formal.}

%We hope that
%our work paves the way for attacking the other variants of \textit{online}
%degree-bounded network design problems as well.\hrnote{mention our lower bound}

%\vlnote{maybe somewhere I should say this problem has mixed packing and coverin constraints. Not sure where though.}

\subsection{Our Contributions}
In the online variant of \dbsf{}, we are given the graph $G$ in advance,
however, demands arrive in an online fashion. At online step $i$, a new
demand $(s_i,t_i)$ arrives. Starting from an empty subgraph, at each step the
online algorithm should augment its solution so that the endpoints of the new
demand $s_i$ and $t_i$ are connected. The goal is to minimize the maximum
degree of the solution subgraph. In the \textit{non-uniform} variant of the
problem, a degree bound $b_v\in \mathbb{R}^+$ is given for every vertex $v$.
For a subgraph $H$ and a vertex $v$, let $\deg_H(v)$ denote the degree of $v$
in $H$. The \textit{load} of a vertex is defined as the ratio
${\deg_H(v)}/{b_v}$. In the non-uniform variant of \odbsf{}, the goal is to
find a subgraph satisfying the demands while minimizing the maximum load of a
vertex.

Our algorithm is a simple and intuitive greedy algorithm. Upon the arrival of a
new demand $(s_i,t_i)$, the greedy algorithm (GA) satisfies the demand by
choosing an $(s_i,t_i)$-path $P_i$ such that after augmenting the solution with
$P_i$, the maximum load of a vertex in $P_i$ is minimum. 
%\hrnote{However, in choosing a
%``\textit{path}'' one should be careful to short-cut through connected
%components of the solution of the previous step. It is not hard to design an
%algorithm similar to Dijkstra's for finding such a path.}\hrnote{Should we
%delete this sentence; } 
A main result of our
paper is to prove that the maximum load of a vertex in the output of GA is
within a logarithmic factor of $\OPT$, the maximum load of a vertex in an
optimal offline solution which knows all the demands in advance.

\begin{theorem}\label{thm:mainlog}
	The algorithm GA produces an output with maximum load at most
	$O(\log n)\cdot \OPT$.
	%  There exists an online algorithm such that the maximum load of a vertex in
	%  the final output is at most $(28\g n +16)\OPT$.
\end{theorem}

The crux of our analysis is establishing several structural properties of the
solution subgraph. First we group the demands according to the maximum load of
the bottleneck vertex at the time of arrival of the demand. We then show that
for every threshold $r>0$, vertices with load at least $r$ at the end of the
run of GA, form a cut set that well separates the group of demands with load at
least $r$ at their bottleneck vertex. Since the threshold value can be chosen
arbitrarily, this leads to a series of cuts that form a chain. The greedy
nature of the algorithm indicates that each cut highly disconnects the demands.
Intuitively, a cut that highly disconnects the graph (or the demands) implies a
lower bound on the number of branches of every feasible solution.

We use a natural dual-fitting argument to show that for every cut set, the
ratio between the number of demands in the corresponding group, over the total
degree bound of the cut, is a lower bound for $\OPT$. Hence, the problem comes
down to showing that one of the cuts in the series has ratio at least $1/O(\log
n)$ fraction of the maximum load $h$ of the output of GA. To this end, we first
partition the range of $r\in (0,h]$ into $O(\log n)$ layers based on the total
degree bound of the corresponding cut. We then show that the required cut can
be found in an interval with maximum range of $r$. We analyze GA formally in
Section~\ref{sec:sfalg}.

We complement our first theorem by giving an example for a special case of
\odbst{} in which no online (randomized) algorithm can achieve a competitive
ratio better than $\Omega(\log n)$.

\begin{theorem}\label{thm:LBst}
	Any (randomized) online algorithm for the degree bounded online Steiner tree
	problem has (multiplicative) competitive ratio $\Omega(\log n)$. This already holds when $b_v=1$
	for every node.
\end{theorem}

We further investigate the following extensions of the online degree bounded
Steiner tree problem. 
First, we
consider the edge-weighted variant of the degree-bounded Steiner tree problem.
Second, we consider the group Steiner tree version in
which each demand consists of a subset of vertices, and the goal is to
find a tree that covers at least one vertex of each demand group. 
The following theorems show that one cannot obtain a non-trivial competitive
ratio for these versions in their general form.\footnote{Our lower bound results imply that one needs
  to restrict the input in order to achieve competitiveness. In particular for
  the edge-weighted variant, our proof does not rule out the existence of a
  competitive algorithm when the edge weights are polynomially bounded. 
%In
%  fact, in the celebrated work of Buchbinder and Naor~\cite{BN09} on online
%  packing/covering LPs, it has been observed before that a log factor of the
%  maximum weight might appear in the competitive ratio of online algorithms for
%  problems with packing constraints.
}



%\bigskip
%\hrule
%\bigskip
% 
% 
%We further ivestigate the online degree-bounded network design problem under
%the following two restrictions.
%online degree-bounded network design problems under
%the following two restrictions. First, we consider the group Steiner tree
%version in which each demand is in the form of a subset of vertices. The goal
%is to find a tree that covers at least one vertex of each demand group. Second,
%we consider the edge-weighted variant of the degree-bounded Steiner tree
%problem. In the following theorem, we show strong lower bounds for both
%problems. One cannot obtain a non-trivial competitive ratio for these problems
%in their general form.

\begin{theorem}\label{thm:ewLB}
Consider the edge weighted variant of \odbst{}. For any (randomized) online
algorithm $\Mc{A}$, there exists an instance and a request sequence such that 
either $\ex{\operatorname{maxdegree}(\Mc{A})}\ge\Omega(n)\cdot b$ or
$\ex{\operatorname{weight}(\Mc{A})}\ge\Omega(n)\cdot \OPT_b$, where $\OPT_b$ denotes
the minimum weight of a Steiner tree with maximum degree $b$.
% 
%  In the edge-weighted variant of \odbst{}, no online (randomized) algorithm
%  can achieve a competitive ratio $o(n)$ for both degree bound and total
%  weight. \hrnote{what does this mean?}
\end{theorem}

\begin{theorem}\label{thm:gstLB}
  There is no deterministic algorithm with competitive ratio $o(n)$ for the
  {\sc degree-bounded group Steiner tree} problem.
% \hrnote{if the set of possible groups
%  is not known in advance.} \hrnote{I would like to delete this portion}
\end{theorem}




\subsection{Related Degree-Bounded Connectivity Problems}\label{sec:related}
The classical family of degree-bounded network design problems have various
applications in broadcasting information, package distribution, decentralized
communication networks, etc.~(see e.g.\
\cite{garcia1988implementation,huang2003publish}). Ravi~\textit{et
  al.}~(\cite{MRSR98},~J. Algorithms'98), first considered the general
\textit{edge-weighted} variant of the problem. They give a bi-criteria $(O(\log
n), O(\log n)\cdot b)$-approximation algorithm, i.e., the degree of every node
in the output tree is $O(\log n)\cdot b$ while its total weight is $O(\log
n)$ times the optimal weight. A long line of work~(see e.g.
\cite{KR00},~STOC'00 and \cite{KR05},~SIAM J. C.) was focused on this problem
until a groundbreaking breakthrough was obtained by
Goemans~(\cite{G06},~FOCS'06); his algorithm computes a minimum-weight spanning
tree with degree at most $b+2$. Later on, Singh and Lau~(\cite{LS07},~STOC'07)
improved the degree approximation factor by designing an algorithm that outputs
a tree with optimal cost while the maximum degree is at most $b+1$.

In the \textit{degree-bounded survivable network design} problem, a number
$d_i$ is associated with each demand $(s_i, t_i)$. The solution subgraph should
contain at least $d_i$ edge-disjoint paths between $s_i$ and $t_i$. Indeed this
problem has been shown to admit bi-criteria approximation algorithms with
constant approximation factors~(e.g. \cite{LS13},~STOC'08). We refer the reader to a recent survey in
\cite{lau2011iterative}. This problem has been recently considered in the
node-weighted variant too (see e.g. \cite{N12,EV14}). The degree-bounded
variant of several other problems such as $k$-MST and $k$-arborescence has also
been considered in the offline setting for which we refer the reader to
\cite{KKN13,BKN09} and references therein.



\subsection{Related Online Problems}
Online network design problems have attracted substantial attention in the last
decades. The online edge-weighted Steiner tree problem, in which the goal is to
find a minimum-weight subgraph connecting the demand nodes, was first
considered by Imase and Waxman~(\cite{IW91},~SIAM J. D. M.'91). They showed
that a natural greedy algorithm has a competitive ratio of $O(\log n)$, which
is optimal up to constants. This result was generalized to the online
edge-weighted Steiner forest problem by Awerbuch \textit{et
  al.}~(\cite{AAB96},~SODA'96) and Berman and Coulston~(\cite{BC97},~STOC'97).
Later on, Naor, Panigrahi, and Singh~(\cite{NPS11}),~FOCS'11) and Hajiaghayi,
Liaghat, and Panigrahi~(\cite{HLP13},~FOCS'13), designed poly-logarithmic
competitive algorithms for the more general \textit{node-weighted} variant of
Steiner connectivity problems. This line of work has been further investigated
in the prize-collecting version of the problem, in which one can ignore a
demand by paying its given penalty. Qian and Williamson~(\cite{QW11},~ICALP'11)
and Hajiaghayi, Liaghat, and Panigrahi~(\cite{HLP14},~ICALP'14) develop
algorithms with a poly-logarithmic competitive algorithms for these variants.

The online $b$-matching problem is another related problem in which
vertices have degree bounds but the objective is to maximize the size of the
solution subgraph. In the worst case model, the celebrated result of Karp
\textit{et al.}~(\cite{KVV90},~STOC'90) gives a $(1-1/e)$-competitive
algorithm. Different variants of this problem have been extensively studied in
the past decade, e.g., for the random arrival model see
\cite{FMMM09,KMT11,MY11,MSVV07}, for the full information model see
\cite{MOS12,MOZ12}, and for the prophet-inequality model see
\cite{AHL11,AHL12,AHL13}. We also refer the reader to the comprehensive
survey by Mehta~\cite{M12}.


Many of the problems mentioned above can be described with an online packing or
covering linear program. Initiated by work of Alon \textit{et
  al.}~\cite{AAABN09} on the online set cover problem, Buchbinder and Naor
developed a strong framework for solving packing/covering LPs fractionally
online. For the applications of their general framework in solving numerous
online problems, we refer the reader to the survey in \cite{BN09}. Azar
\textit{et al.}~\cite{ABFP13} generalize this method for the fractional
\textit{mixed} packing and covering LPs. In particular, they show an
application of their method for integrally solving a generalization of
capacitated set cover. Their result is a bi-criteria competitive algorithm that
violates the capacities by at most an $O(\log^2 n)$ factor while the cost of
the ouput is within $O(\log^2 n)$ factor of optimal.
We note that although the fractional variant of our problem is a special case of online mixed packing/covering LPs, we do not know of any online rounding method for Steiner connectivity problems.

\subsection{Preliminaries}
Let $G=(V, E)$ denote an undirected graph of size $n$ ($|V|=n$). For every
vertex $v\in V$, let $b_v\in \mathbb{R}^+$ denote the \textit{degree bound} of
$v$. In the \dbsf{} problem, we are given a sequence of connectivity
\textit{demands}. The $i^{th}$ demand is a pair of vertices $(s_i,t_i)$ which
we call the \textit{endpoints} of the demand. An algorithm outputs a subgraph
$H\subseteq G$ in which for every demand its endpoints are connected. The
\textit{load} of a vertex $v$ w.r.t. $H$ is defined as
$\ell_H(v)={\deg_H(v)}/{b_v}$. We may drop the subscript $H$ when it is clear
from the context. The goal is to find a subgraph $H$ that minimizes the maximum
load of a vertex. Observe that one can always find an optimal solution without
a cycle, hence the name Steiner \textit{forest}. Furthermore, without loss of
generality\footnote{One can add a dummy vertex for every vertex $v\in V$
  connected to $v$. We then interpret a demand between two vertices as a demand
  between the corresponding dummy vertices. The degree bound of a dummy vertex
  can be set to infinity. This transformation can increase the degree of any
  node by at most a factor of $2$, which does not affect our asymptotic
  results.}, we assume that the endpoints of the demands are distinct vertices
with degree one in $G$ and degree bound infinity. We denote the maximum load of
a vertex in an optimal subgraph by $\OPT=\min_{H} \max_{v} \ell_H(v)$.

The following mixed packing/covering linear program (\ref{LP:sf}) is a
relaxation for the natural integer program for \dbsf{}. Let $\Mc{S}$ denote the
collection of subsets of vertices that separate the endpoints of at least one
demand. For a set of vertices $S$, let $\delta(S)$ denote the set of edges with
exactly one endpoint in $S$. In \ref{LP:sf}, for an edge $e$, $\x(e)=1$
indicates that we include $e$ in the solution while $\x(e)=0$ indicates
otherwise. The variable $\alpha$ indicates an upper bound on the load of every
vertex. The first set of constraints ensures that the endpoints of every demand
is connected. The second set of constraints ensures that the load of a vertex is
upper bounded by $\alpha$. The program \ref{LP:dualsf} is the dual of the LP
relaxation \ref{LP:sf}.

\def\myrule{\phantom{\rule[-3.2ex]{1pt}{5.6ex}}}
\noindent
\begin{minipage}{.44\textwidth} %
\begin{align*}
\text{minimize}           &\quad \myrule\alpha \tag{{$\mathbb{P}$}}\label{LP:sf}\\
\forall S\subseteq \Mc{S} &\quad \myrule\zsum{e\in \delta\smash{(S)}}{\x(e)} \geq 1 \tag{$\y(S)$}\\
\forall v\in V            &\quad \myrule\zsum{e\in \delta\smash{(\{v\})}}{\x(e)} \leq \alpha \cdot b_v \tag{$\z(v)$} \\
                          &\quad \myrule\x(e), \alpha\in \mathbb{R}_{\geq 0} 
\end{align*}
\end{minipage} %
\hspace{0.02\textwidth}
\begin{minipage}{.53\textwidth} %
\begin{align*}
\text{maximize} &\quad  \myrule\zsum{S\in \Mc{S}}{\y(S)} \tag{{$\mathbb{D}$}}\label{LP:dualsf}\\
\forall e=(u,v) &\quad  \myrule\zsum{S: e\in \delta\smash{(S)}}{\y(S)} \leq \z(u)+\z(v) \tag{$\x(e)$}\\
                &\quad  \myrule\zsum{v}{\z(v)b_v} \leq 1 \tag{$\alpha$} \\
                &\quad  \myrule\z(v), \y(S)\in \mathbb{R}_{\geq 0}
\end{align*}
\end{minipage}
In the online variant of the problem, $G$ and the degree bounds are known in
advance, however, the demands are given one by one. Upon the arrival of the
$i^{th}$ demand, the online algorithm needs to output a subgraph $H_i$ that
satisfies all the demands seen so far. The output subgraph can only be
augmented, i.e., for every $j<i$, $H_j\subseteq H_i$. The \textit{competitive
  ratio} of an online algorithm is then defined as the worst case ratio of
${\max_v \ell_{H}(v)}/{\OPT}$ over all possible demand sequences where
$H$ is the final output of the algorithm.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "notes"
%%% End: 

==> draft (1)/weighted.tex <==
\subsection{{\sc Online Degree-Bounded Edge-weighted Steiner Tree}}
Below we present a graph instance $G=(V,E)$ for online bounded-degree
edge-weighted Steiner tree in which for any (randomized) online algorithm $A$
there exists a demand sequence for which $A$ either violates the degree bound
by a large factor or generates a much larger weight than the optimum.

%\iffalse with edges of exponential weight\fi in
%which no online (randomized) algorithm can simultaneously meet both degree and
%weight bounds with any competitive ratio of $o(n)$ i.e. any online (randomized)
%algorithm would in average violate degree and/or weight bounds by a ratio of
%$\Omega(n)$.

Consider a graph $G$ as shown in Figure~\ref{fig:1}, which has $n=2k+1$ nodes
and $3k$ edges. Every node $i$ ($1\leq i\leq k$) is connected to the root with
a zero-weight edge and to node $k+i$ with weight $n^i$. In addition, there
exist zero-weight edges connecting node $i$ ($k+1 \leq i < 2k$) to node $i+1$,
and there exists a zero-weight edge that connects node $2k$ to the root.
 We assume that all node weights $b_v$ are equal to one and the degree bound $b$
 for $\OPT$ is equal to $3$.
\begin{figure*}[!h]
	\centering
	
	\begin{subfigure}[b]{0.44\textwidth}
		\includegraphics[width=\textwidth]{fig1.pdf}
		\caption{The graph $G$ consists of $2k+1$ nodes and $3k$ edges.}
		\label{fig:1}
	\end{subfigure}%
	\hspace{0.1\textwidth}
	\begin{subfigure}[b]{0.44\textwidth}
		\includegraphics[width=\textwidth]{fig2.pdf}
		\caption{The highlighted subtree represents an optimum solution $\OPT_3$.}
		\label{fig:2}
	\end{subfigure}%
	\caption{The hard example for edge-weighted Steiner tree}
\end{figure*}

\begin{proof}[of Theorem~\ref{thm:ewLB}]
%  In order to prove the theorem, we present an order for the adversary to give
%  terminals in graph $G$ such that any online (randomized) algorithm $A$ fails
%  to achieve a competitive ratio of $o(n)$ for both degree and weight bounds.
%  The order is as follows:
  The adversary consecutively presents terminals starting from node $1$. At
  each step $i$ the algorithm $A$ adds some edges to its current solution
  such that the $i^{th}$ terminal $t_i=i$ gets connected to the $\mathit{root}$.

  We use $X_i$ to denote the subset of edges chosen by $A$ after step $i$. We also use
  $0\leq p_{ij}\leq 1$ and $0\leq q_{ij}\leq 1$ to denote the probability that
  the edges $\{i,\mathit{root}\}$ and $\{i,k+i\}$, respectively, are in $X_j$ . After each
  step $j$, all terminals $t_i$ ($i\leq j$) must be connected to the $\mathit{root}$ by
  at least one of $\{i,\mathit{root}\}$ or $\{i,k+i\}$. Therefore $p_{ij}+q_{ij}\geq 1$.
  In addition, for every $j_1\leq j_2$ we have $q_{ij_1}\leq q_{ij_2}$ and
  $p_{ij_1}\leq p_{ij_2}$, because $X_{j_1} \subseteq X_{j_2}$.
  The adversary stops the sequence at the first step $r$ for which $q_{rr}>{1}/{2}$.
  If this never happens the sequence is stopped after requesting $k$ nodes.

%, if and only if $q_{rr}$ is more than
%  $\frac{1}{2}$. Otherwise it will go ahead to step $k$.

  We use $\OPT_b$ to denote the weight of a minimum Steiner tree with maximum
  degree $b=3$. In order to find an upper bound for $\OPT_b$, consider the
  following tree $T$:
\begin{align*}
T&=\{\{i,k+i\}|1\leq i\leq r-1\} \cup \{\{i,i+1\}|k\leq i<2k\} \cup \{\{2k,\mathit{root}\},\{r,\mathit{root}\}\}\enspace.
\end{align*}
As we can observe in Figure~\ref{fig:2}, $T$ meets the degree bounds and
connects the first $r$ terminals to the root, so forms a valid solution. We have
\begin{equation*}
w(\OPT) \leq w(T)=\sum_{i=1}^{r-1} n^i \in O(n^{r-1})\enspace.
\end{equation*}

\noindent
Back to algorithm $A$, the adversary causes one of the following two
cases: 
\begin{enumerate}[leftmargin=*,label=(Case~\alph*)]
\item
The process stops at step $r$ with
$q_{rr}>\frac{1}{2}$. Then
\begin{align*}
\ex[w(X_r)]&=\sum_{i=1}^{r} q_{ir}\cdot n^i \geq q_{rr}\cdot n^r\geq \frac{n^r}{2}\enspace.
\end{align*}
Hence, $\ex[w(X)]\ge\Omega(n)\cdot w(\OPT)$.
%&\Rightarrow \frac{E[w(X)]}{w(\OPT)} \in \Omega(n)
\item
The process continues until step $k$, i.e., for every $i\leq k$, $q_{ii}\leq\frac{1}{2}$.
\begin{align*}
\ex[\operatorname{deg}(\mathit{root})] 
&\ge\sum_{i=1}^{k}p_{ik}\ge\sum_{i=1}^{k}p_{ii}\geq\sum_{i=1}^{k}(1-q_{ii})\ge\frac{k}{2}=\frac{n-1}{4}\enspace.
\end{align*}
Hence, $\ex[\operatorname{deg}(\mathit{root})]\ge  \Omega(n)\cdot b$.
\end{enumerate}
This shows that for any online algorithm $A$ there is a demand sequence on
which $A$ either generates a large weight or violates the degree bound by a
large factor.
% 
% 
%Above shows that any online (randomized) algorithm $A$ would be trapped in
%either of the cases $i$ or $ii$, and thus cannot achieve a competitive ratio of
%$o(n)$ for both degree and weight bounds.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "notes"
%%% End: 
